Stability Analysis of Inline ZFP Compression for Floating-Point Data in Iterative Methods

Currently, the dominating constraint in many high performance computing applications is data capacity and bandwidth, in both inter-node communications and even more-so in on-node data motion. A new approach to address this limitation is to make use of data compression in the form of a compressed data array. Storing data in a compressed data array and converting to standard IEEE-754 types as needed during a computation can reduce the pressure on bandwidth and storage. However, repeated conversions (lossy compression and decompression) introduce additional approximation errors, which need to be shown to not significantly affect the simulation results. We extend recent work [J. Diffenderfer, et al., Error Analysis of ZFP Compression for Floating-Point Data, SIAM Journal on Scientific Computing, 2019] that analyzed the error of a single use of compression and decompression of the ZFP compressed data array representation [P. Lindstrom, Fixed-rate compressed floating-point arrays, IEEE Transactions on Visualization and Computer Graphics, 2014] to the case of time-stepping and iterative schemes, where an advancement operator is repeatedly applied in addition to the conversions. We show that the accumulated error for iterative methods involving fixed-point and time evolving iterations is bounded under standard constraints. An upper bound is established on the number of additional iterations required for the convergence of stationary fixed-point iterations. An additional analysis of traditional forward and backward error of stationary iterative methods using ZFP compressed arrays is also presented. The results of several 1D, 2D, and 3D test problems are provided to demonstrate the correctness of the theoretical bounds.

==> compression.tex <==
\section{ZFP Data Compression}
\label{sec:zfp}
We first provide a brief overview of the current ZFP compression algorithm. Further details of the implementation of ZFP can be found in \cite{zfp} with modifications described in the software documentation \cite{zfp-doc}.
 \begin{itemize}
\item[\it Step 1:]The $d$-dimensional array is partitioned into arrays of dimension $4^d$, called \emph{blocks}. A 2-d example is depicted in Figure \ref{fig:cut4dblock}. If the $d$-dimensional array cannot be partitioned exactly into blocks, then the boundary of the $d$-dimensional array is padded until an exact partition is possible.
\begin{figure}
    \centering
        \includegraphics[width=.45\textwidth]{figures/step1.pdf}
    \caption{Deconstruction of a 2-dimensional array into independent $4\times4$ blocks. If the data is not divisible by 4 the data at the boundaries is padded (shown in orange).}
    \label{fig:cut4dblock}
\end{figure}
\begin{figure}
    \centering
        \includegraphics[width=.8\textwidth]{figures/step3.pdf}
    \caption{Floating-point bit representation in single precision converted to a block-floating-point representation and its corresponding signed integers. Note that, depending on the relative disparity of the 16 numbers, some truncation may occur for the numbers of the smallest magnitude. }
   \label{fig:bfprepresentation}
\end{figure}
\item[\it Step 2:] The floating-point values in each block are converted
  to a block-floating-point representation using a common exponent for
  each block \cite{MitrablockRoundingError} and integers in two's complement
  format. The block-floating point representation is then shifted and
  rounded to $4^d$ signed integers as seen in Figure
  \ref{fig:bfprepresentation}. 
\item[\it Step 3:]The integers are decorrelated using a custom, high-speed, near orthogonal transform that is similar to the discrete cosine transform; see Section \ref{Step3Sec} for details.
\item[\it Step 4:] The signed integer coefficients are reordered by total sequency (See \cite{zfp-doc} for details). A 2-d example can be seen in Figure \ref{fig:totalsequency}. 
\begin{figure}
    \centering
        \includegraphics[width=.5\textwidth]{figures/step4.pdf}
    \caption{Total sequency ordering for a 2-dimensional array, which groups the diagonal elements together. }
    \label{fig:totalsequency}
\end{figure}
\item[\it Step 5:] The two's complement signed integers (the standard
  integer representation) are converted to their negabinary
  representation~\cite{Knuth}.  
\item[\it Step 6:] The bits that represent the list of $4^d$ integers
  are transposed so that they are ordered by bit plane, from most to
  least significant bit, instead of by coefficient.  
\item[\it Step 7:] Each bit plane is compressed losslessly using
  embedded coding, which exploits the property that the transform
  coefficients tend to have many leading zeros. As this step is
  lossless, the encoding details are omitted.  
\item[\it Step 8:]The embedded coder emits one bit at a time until
  stopping criteria are satisfied. The exact stopping criteria is dependent on the mode of ZFP compression: either fixed rate, fixed precision, or
  fixed accuracy.   
\end{itemize}

Most of our discussion and error analysis in Section~\ref{sec:analysis}
will focus on Steps 2, 3, and 8 as these steps are likely to introduce
additional round-off error during compression and, in some cases, during
decompression. Our approach for bounding the round off error introduced
by ZFP compression and decomporession is to define an operator for each
step of the algorithm, compose these operators to form a ZFP compression
and a ZFP decompression operator, compute the value returned after
compressing and decompressing an arbitrary input, and finally compare
this value to the value of the original input. The next section will
focus on introducing notation and definitions that will be useful in
defining mathematical operators for each step of the ZFP compression
algorithm.   
%For reference, Table \ref{table:notation} briefly describes the notation used and the section and/or equation in which it is defined. 
\renewcommand\arraystretch{1.2}
\begin{table}[htp!]
\caption{Notation Table} 
\begin{center}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|c l c|}
\hline 
Symbol & Description & Location \\
\hline 
\hline
$\cI$ & active bit set & \S \ref{sec:notation}  \\
%$\cB$ & infinite bit space & \S \ref{sec:bitvectorSpace} \\
$\cB^n$ & infinite binary vector space & \S \ref{sec:bitvectorSpace} \\
$\cB^n_k$ & subset of $\cB^n$ with finite active bit set & \S \ref{sec:bitvectorSpace} \\
$\cN^n$ & infinite negabinary vector space & \S  \ref{sec:bitvectorSpace}\\
$\cN_k^n$ & subset of $\cN^n$ with finite active bit set & \S \ref{sec:bitvectorSpace}\\
$\bf{0}_\cB$,$\bf{0}_\cN$  & additive identity in $\cB^n$ and $\cN^n$, respectively & \S \ref{sec:bitvectorSpace}\\ 
$\bf{1}_\cB $, $\bf{1}_\cN$  & multiplicative identity in $\cB^n$ and $\cN^n$, respectively & \S \ref{sec:bitvectorSpace}\\
$\| \cdot \|_{\cB, p}$, $\| \cdot \|_{\cN, p}$  & $p$-norm with respect to $\cB^n$ and $\cN^n$, respectively & \S \ref{NormsSubsection} \\

\hline
$f_\cB$, $f_\cB^{-1}$, $f_\cN$, $f_\cN^{-1}$ & bijective maps from $\cB \rightarrow \mathbb{R}$, $\mathbb{R} \rightarrow \cB$, $\cN \rightarrow \mathbb{R}$ and $\mathbb{R} \rightarrow \cN$, respectively & Eqn. (\ref{eqn:f2})\\
$F_\cB$,$F_\cB^{-1}$ & bijective maps from $\cB^n \rightarrow \mathbb{R}^n$ and $\mathbb{R}^n \rightarrow \cB^n$, respectively & Eqn. (\ref{eqn:F2})\\
$F_{\cN}$,$F_\cN^{-1}$  & bijective maps from $\cN^n \rightarrow \mathbb{R}^n$ and $\mathbb{R}^n \rightarrow \cN^n$, respectively & Eqn. (\ref{eqn:FN})\\

$\oplus $ &bit vector addition  & Lma. \ref{FieldLemma}\\
$\odot$ &bit vector multiplication & Lma. \ref{FieldLemma}\\
\hline

$s_l$, $S_l$ & shift operator on $\cB$ and $\cB^n$, respectively & \S \ref{ShiftSubsection} \\
$t_{\cS_k},T_{\cS_k} $ & truncation operator with respect to the set $\cS_k$ & \ref{DefCOperators} \\
{$r $} & rounding operator for two's complement representation & \S \ref{Step3Sec} \\
$e_{min}$, $e_{max}$ & min and max exponent of the floating-point representation of the block &  Def.  \ref{def:emaxemin}\\
$\epsilon_m$ & constant $\epsilon_m := 2^{1-m}$, with $m \in \mathbb{N}$ &  \S \ref{sec:bitvectorSpace} \\
\hline
$L$, $L_d$ & one and $d$-dimension forward decorrelating linear transform &  Eqn.   \ref{eqn:T} \\
$\tilde{L}$, $\tilde{L}_d$ & floating-point arithmetic approximation of $L$ and $L_d$ &  \S \ref{Step3Sec}   \\
$L_d^{-1} $,  $\tilde{L}^{-1} _d$ &  $d$-dimension backward decorrelating linear transform and the floating-point arithmetic approximation of $L^{-1}$&  \S \ref{Step3Sec} \\
\hline
$C_k$, $\tilde{C_k}$ & lossless/lossy operator for Step $k$ of ZFP compression & \S \ref{sec:analysis} \\
%$C_2$, $\tilde{C_2}$ & lossless/lossy compression operator of Step 2 (block-floating-point) &\S \ref{Step2Sec}\\
%$C_3$, $\tilde{C_3}$ & lossless/lossy compression operator of Step 3 (decorrelating transform)&  \S \ref{Step3Sec} \\
%$C_8$, $\tilde{C_8}$ &lossless/lossy compression operator of Step 8 (bit-plane approximation)&  \S  \ref{Step78Sec}  \\
%\hline
$D_k$, $\tilde{D_k}$ & lossless/lossy operator for Step $k$ of ZFP decompression & \S \ref{sec:analysis} \\
%$D_3$, $\tilde{D_3}$ & lossless/lossy decompression operator of Step 3 (decorrelating transform)&   \S \ref{Step3Sec} \\
\hline
\end{tabular}
\end{adjustbox}
\end{center}

\label{table:notation}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> notation.tex <==
\section{Preliminary Notations, Definitions, and Lemmas}
\label{sec:notation}
%%\subsection{Definition of the Two's Complement Bit-Vector Space}
%\label{IntroSec:seqspace} 
%As noted in the outline of the ZFP compression algorithm in Section
%\ref{sec:zfp}, many of the steps of ZFP are defined by direct
%manipulation of the bits used to represent each component of the
%input. While we could attempt to define operators that imitate the steps
%of ZFP over the real vector space, it would be more straightforward to
%work with the bitwise representation that is manipulated at each step of
%the ZFP compression algorithm. Hence, in order to define operators for
%each step of ZFP as actions on the bitwise representation of each
%component, we construct vector spaces under which the components
%correspond to binary or negabinary representations of the real
%numbers. Accordingly, let $\mathbb{B} = \{ 0, 1 \}$ and define  
%\begin{align}
%\mathcal{C} := \left\{ \{ c_i \}_{i = -\infty}^{\infty} : c_i \in \mathbb{B} \ \text{for all} \ i \in \mathbb{Z} \right\} \label{eqn:infinitebitvector}.
%\end{align}
%For an element $c \in \mathcal{C}$, we define the \emph{active bit set of
%  $c$} by $\mathcal{I} (c) := \{ i \in \mathbb{Z} : c_i = 1 \}.$
%Additionally, we define the following operators on $\mathcal{C}$ that
%will be used as building blocks for defining each step of ZFP. 
%\begin{definition}\label{DefCOperators}
%Let $\mathcal{S} \subseteq \mathbb{Z}$. The \emph{truncation operator},
%$t_{\mathcal{S}} : \mathcal{C} \to \mathcal{C}$,  is defined by  
%\begin{align*}
%t_{\mathcal{S}} (c)_i = \left\{ \begin{array}{ccc} 
%                c_i &: & i \in \mathcal{S} \\
%                0 &: & i \not\in \mathcal{S} \\
%                \end{array} \right., \ \ \ \text{for all} \ c \in \mathcal{C} \ \text{and all} \ i \in \mathbb{Z}.
%\end{align*}
%Let $\ell \in \mathbb{Z}$. The \emph{shift operator}, $s_{\ell} :
%\mathcal{C} \to \mathcal{C}$, is defined by 
%\begin{align*}
%s_{\ell} (c)_i = c_{i + \ell}, \ \ \ \text{for all} \ c \in \mathcal{C} \ \text{and all} \ i \in \mathbb{Z}.
%\end{align*}
%\end{definition}
%\noindent From these definitions, it follows that $t_{\mathcal{S}}$ is a
%nonlinear operator and that $s_{\ell}$ is a linear operator. These operators
%can be extended to operators on $\mathcal{C}^n$. Accordingly,
%$T_{\mathcal{S}} : \mathcal{C}^n \to \mathcal{C}^n$ is defined by 
%%\aedit{Let $\bc \in \mathcal{C}^n$ be a vector of infinite bit vectors. Let $\bc_i \in \mathcal{C}$ for all $i =1,\dots,n$ be the $i$-th element in $\bc$, where $\bc_i$ is a bit vector defined by (\ref{eqn:infinitebitvector}), and let $\bc_{i,l} = (\bc_i)_l \in \mathbb{B} $ for all $l\in \mathbb{Z}$ be the $l$-th binary element of bit vector $\bc_i$. The above notation will be used for all vectors of infinite bit vectors no matter the binary representation.}
%
%\begin{align*}
%T_{\mathcal{S}} (\bm{c}) = \begin{bmatrix}
%\ t_{\mathcal{S}} ({\bc}_1) \ \\
%\ \vdots \ \\
%\ t_{\mathcal{S}} ({\bc}_n) \ \
%\end{bmatrix}, \ \text{for all} \ \bm{c} = \begin{bmatrix}
%\ {\bc}_1 \ \ \\
%\ \vdots \ \ \\
%\ {\bc}_n \ \
%\end{bmatrix}  \in \mathcal{C}^n,
%\end{align*}
%and we define $S_{\ell} : \mathcal{C}^n \to \mathcal{C}^n$ by 
%\begin{align*}
%S_{\ell} (\bc) = \begin{bmatrix}
%\ s_{\ell} ({\bc}_1) \ \\
%\ \vdots \ \\
%\ s_{\ell} ({\bc}_n) \ \
%\end{bmatrix} \text{, for all }\bm{c} = \begin{bmatrix}
%\ \bc_1 \ \ \\
%\ \vdots \ \ \\
%\ {\bc}_n \ \
%\end{bmatrix} \in \mathcal{C}^n.
%\end{align*}
%For clarity, note that the components $\bc_1, \ldots, \bc_n$ of $\bm{c} = \left[ \bc_1, \ \cdots, \ \bc_n \right]^t \in \mathcal{C}^n$ are each binary sequences as $\bc_i \in \mathcal{C}$ for $1 \leq i \leq n$. Additionally, note that $S_{\ell}$ is invertible with $S_{\ell}^{-1} : \mathcal{C}^n \to \mathcal{C}^n$ given by $S_{\ell}^{-1} = S_{-\ell}$. 
%
%\subsection{Defining Signed Binary and Negabinary Bit-Vector Spaces}
%\label{sec:bitvectorSpace}
%Let $x \in \mathbb{R}$  be given. Then there exist elements $c, d \in \mathcal{C}$ and $p \in \mathbb{B}$ such that $x$ can be represented in in signed binary and negabinary as 
%\begin{align}
%{\text{Signed Binary: }} x = (-1)^p \sum_{i = - \infty}^{\infty} c_i 2^i \ \ \ \text{ and}  \ \ \ {\text{ Negabinary: }} x = \sum_{i = - \infty}^{\infty} d_i (-2)^i. \label{CrepX}
%\end{align}
%As such, there exist subsets $\mathcal{A}$ and $\mathcal{N}$ of
%$\mathcal{C}$ such that, for each $x \in \mathbb{R}$, there exist unique
%elements $c \in \mathcal{A}$, $p \in \mathbb{B}$, and $d \in
%\mathcal{N}$ such that $x$ can be represented in the binary and
%negabinary form in (\ref{CrepX}) using $c$, $p$, and $d$,
%respectively. In particular, we choose $\mathcal{A}$ and $\mathcal{N}$
%such that $\mathcal{I} (c)$ and $\mathcal{I} (d)$ are finite whenever
%possible. This choice is made so that elements, such as the integers,
%can be represented using finitely many nonzero bits. Now define
%$0_{\mathcal{C}}, 1_{\mathcal{C}} \in \mathcal{C}$ to be the elements
%satisfying $\mathcal{I} \left( 0_{\mathcal{C}} \right) = \emptyset$ and
%$\mathcal{I} \left( 1_{\mathcal{C}} \right) = \{ 0 \}$. It follows from
%our choice of $\mathcal{A}$ and $\mathcal{N}$ that $\left\{
%0_{\mathcal{C}}, 1_{\mathcal{C}} \right\} \subset \mathcal{A} \cap
%\mathcal{N}$.  
%
%Defining $\mathcal{B} := \{ (p, a) \in  \mathbb{B} \times \mathcal{A} :
%(p, a) \neq ( 1, 0_{\mathcal{C}} ) \}$, we have that, for each $x \in
%\mathbb{R}$, there exists a unique $b = (p, a) \in \mathcal{B}$ such that
%$x = (-1)^p \sum_{i = - \infty}^{\infty} a_i 2^i$. Additionally, it is
%clear from our choice of $\mathcal{N}$ that, for each $x \in \mathbb{R}$,
%there exists a unique $d \in \mathcal{N}$ such that $x = \sum_{i = -
%  \infty}^{\infty} d_i (-2)^i$. We now define $f_\cB : \mathcal{B} \to
%\mathbb{R}$ by 
%\begin{equation}
%\label{eqn:f2}
%f_\cB (b) = (-1)^{{p}} \sum_{i = -\infty}^{\infty} a_i 2^i, \ \ \ \ \ \text{for all} \ b = ({p}, a) \in \mathcal{B},
%\end{equation}
%and $f_\cN : \mathcal{N} \to \mathbb{R}$ by 
%\begin{equation}
%\label{eqn:fN}
%f_\cN (d) = \sum_{i = -\infty}^{\infty} d_i (-2)^i, \ \ \ \ \ \text{for all} \ d \in \mathcal{N}.
%\end{equation}
%By our choice of $\mathcal{B}$ and $\mathcal{N}$, we have that $f_\cB$ and $f_\cN$ are bijections and, hence, are invertible with inverses denoted by $f_\cB^{-1} : \mathbb{R} \to \mathcal{B}$ and $f_\cN^{-1} : \mathbb{R} \to \mathcal{N}$, respectively. Using these functions, we now define the binary operators $\oplus_{\mathcal{B}} : \mathcal{B} \times \mathcal{B} \to \mathcal{B}$ and $\odot_{\mathcal{B}} : \mathcal{B} \times \mathcal{B} \to \mathcal{B}$ by
%\begin{align}
%\alpha \oplus_{\mathcal{B}} \beta= f_\cB^{-1} \left( f_\cB( \alpha ) + f_\cB(\beta) \right) \label{oplusdef}
%\end{align}
%and
%\begin{align}
%\alpha \odot_{\mathcal{B}} \beta = f_\cB^{-1} \left( f_\cB(\alpha) \cdot f_\cB(\beta) \right) \label{otimesdef}, 
%\end{align}
%for all $\alpha, \beta \in \mathcal{B}$, where $+$ and $\cdot$ represent standard addition and multiplication in $\mathbb{R}$. Similarly, we can define $\oplus_{\mathcal{N}} : \mathcal{N} \times \mathcal{N} \to \mathcal{N}$ and $\odot_{\mathcal{N}} : \mathcal{N} \times \mathcal{N} \to \mathcal{N}$ by replacing all $\mathcal{B}$ with $\mathcal{N}$ in (\ref{oplusdef}) and (\ref{otimesdef}). With these definitions in place, we now have the following result.
%
%\begin{lemma}\label{FieldLemma}
%$(\mathcal{B}, \oplus_\mathcal{B}, \odot_\mathcal{B})$ is a field with additive identity $0_{\mathcal{B}} := (0,0_{\mathcal{C}})$ and multiplicative identity $1_{\mathcal{B}} := (0, 1_{\mathcal{C}})$. $(\mathcal{N}, \oplus_\mathcal{N}, \odot_\mathcal{N})$ is a field with additive identity $0_{\mathcal{N}} := 0_{\mathcal{C}}$ and multiplicative identity $1_{\mathcal{N}} := 1_{\mathcal{C}}$.
%\end{lemma} 
%
%For the remainder of the discussion, the sign bit will be omitted from
%elements of $\mathcal{B}$ by letting $a$ represent the element $(0,a)
%\in \mathcal{B}$ and $- a$ represent $(1,a) \in
%\mathcal{B}$. Additionally, we will write $+$ instead of
%$\oplus_{\mathcal{B}}$ or $\oplus_{\mathcal{N}}$ where the operation
%should be clear from the context in which it is used. These choices are
%made to simplify the notation in the following sections.  
%
%
%Next, we note that $f_\cB$ and $f_\cN$ can be generalized to
%vector-valued functions by defining $F_\cB : \mathcal{B}^n \to
%\mathbb{R}^n$ as 
%\begin{equation} \label{eqn:F2}
%F_\cB(\bm{a}) = \begin{bmatrix}
%\ f_\cB({\ba}_1) \ \ \\
%\ \vdots \ \ \\
%\ f_\cB({\ba}_n) \ \
%\end{bmatrix}, \ \text{for all} \ \bm{a} = \begin{bmatrix}
%\ {\ba}_1 \ \ \\
%\ \vdots \ \ \\
%\ {\ba}_n \ \
%\end{bmatrix}  \in \mathcal{B}^n,
%\end{equation} 
%and $F_\cN : \mathcal{N}^n \to \mathbb{R}^n$ as
%\begin{equation}\label{eqn:FN}
%F_\cN ({\bd}) = \begin{bmatrix}
%\ f_\cN({\bd}_1) \ \ \\
%\ \vdots \ \ \\
%\ f_\cN({\bd}_n) \ \
%\end{bmatrix}, \ \text{for all} \ \bm{d} = \begin{bmatrix}
%\ {\bd}_1 \ \ \\
%\ \vdots \ \ \\
%\ {\bd}_n \ \
%\end{bmatrix} \in \mathcal{N}^n.
%\end{equation}
%Note that $F_\cB$ and $F_\cN$ are invertible with inverses $F_\cB^{-1}$ and $F_\cN^{-1}$ defined by applying $f_\cB^{-1}$ and $f_\cN^{-1}$ componentwise, respectively. We will let $\bm{0}_{\mathcal{B}}$ denote the additive identity in $\mathcal{B}^n$ and $\bm{0}_{\mathcal{N}}$ denote the the additive identity in $\mathcal{N}^n$. Similarly, we let $I_{\mathcal{B}} : \mathcal{B}^n \to \mathcal{B}^n$ and $I_{\mathcal{N}} : \mathcal{N}^n \to \mathcal{N}^n$ denote the identity map on $\mathcal{B}^n$ and $\mathcal{N}^n$, respectively.
%
%To imitate floating-point or fixed-point representations used in a computer, we define the following subsets of $\cB$ and $\cN$. Given $k \in \mathbb{N}$, we define 
%\begin{align*}
%\mathcal{B}_{k} := \left\{ (p,a) \in \mathcal{B} : \mathcal{I} (a) \subseteq \{ i, i + 1, \ldots, {i + k -1} \} \ \text{for some} \ i \in \mathbb{Z} \right\}
%\end{align*}
%and
%\begin{align*}
%\mathcal{N}_{k} := \left\{ d \in \mathcal{N} : \mathcal{I} (d) \subseteq \{ i, i + 1, \ldots,  i + k -1 \} \ \text{for some} \ i \in \mathbb{Z} \right\}. 
%\end{align*}
%Here, $k$ represents the maximum number of nonzero bits allotted
%  for each representation. For example, in $\cB_k$, $k$ represents the
%  number of bits allotted for the mantissa in IEEE and $i$ indicates the
%  exponent in IEEE. It should be noted that, for any $k \in
%\mathbb{N}$, $\mathcal{B}_{k}$ and $\mathcal{N}_k$ are subsets but
%\emph{not} subspaces of $\mathcal{B}$ and $\mathcal{N}$, respectively,
%as they do not satisfy the property of closure under $\oplus$ and
%$\odot$. As such, the analysis will take place in either $\cB$, $\cN$,
%or $\mathbb{R}$ with the use of the truncation operator $T_\cS$ to
%imitate working with finite precision elements. 
%
%\subsection{Meaningful Norms on $\mathcal{B}^n$ and $\mathcal{N}^n$}\label{NormsSubsection}
%From Lemma \ref{FieldLemma}, it follows that $\mathcal{B}^n$ is a vector
%space under $+$. As such, we now wish to determine norms $\| \cdot
%\|_{\mathcal{B}, p} : \mathcal{B}^n \to [0, \infty)$ under which
%  $F_{\mathcal{B}} : \mathcal{B}^n \to \mathbb{R}^n$ is an isometry,
%  that is, norms that satisfy $\| F_\cB (\bm{a}) \|_p = \| \bm{a}
%  \|_{\mathcal{B}, p}$, for all $\bm{a} \in \mathcal{B}^n$, where $\|
%  \cdot \|_p$ is the standard $p$-norm on $\mathbb{R}^n$. Accordingly,
%  we define $\| \cdot \|_{\mathcal{B}, p} : \mathcal{B}^n \to [0,
%    \infty)$ by  
%\begin{align}
%\| \bm{a} \|_{\mathcal{B}, p} = \left( \sum_{i = 1}^{n} \left| f_\cB(\bm{a}_i) \right|^{p} \right)^{1/p}, \ \ \ \text{for} \ 1\leq p <\infty, \label{BpNorm}
%\end{align}
%and 
%\begin{align}
%\| \bm{a} \|_{\mathcal{B}, \infty} = \max_{1 \leq i \leq n} \left| f_\cB(\bm{a}_i) \right|. \label{BinfNorm}
%\end{align}
%The following result is an immediate consequence from this definition of $\| \cdot \|_{\mathcal{B}, p}$.
%
%\begin{lemma}
%\label{BNormLemma}
%For all $\bm{a} \in \mathcal{B}^n$, $\bm{x} \in \mathbb{R}^n$, and $1 \leq p \leq \infty$, $\| \cdot \|_{\mathcal{B}, p}$ is a norm satisfying 
%\begin{align*}
%\| F_\cB (\bm{a}) \|_p = \| \bm{a} \|_{\mathcal{B}, p} \ \ \ \text{and} \ \ \ \| \bm{x} \|_p = \| F_\cB^{-1} (\bm{x}) \|_{\mathcal{B}, p}.
%\end{align*}
%\end{lemma}
%\noindent For any $1 \leq p \leq \infty$, we now have that $\mathcal{B}^n$ is a normed vector space with norm $\| \cdot \|_{\mathcal{B}, p}$. Additionally, we can define a norm for operators defined on $\mathcal{B}^n$.
%
%\begin{definition}
%\label{BopNorm}
%Suppose that $\Phi : \mathcal{B}^n \to \mathcal{B}^m$ for $m,n \in \mathbb{N}$. For $1 \leq p \leq \infty$, the induced p-norm on $\Phi$ is defined by
%\begin{align*}
%\| \Phi \|_{\mathcal{B}, p} = \sup \left\{ \frac{\| \Phi (\bm{a}) \|_{\mathcal{B}, p}}{\| \bm{a} \|_{\mathcal{B}, p}} : \bm{a} \in \mathcal{B}^n, \bm{a} \neq \bm{0}_{\mathcal{B}} \right\}.
%\end{align*}
%\end{definition}
%\noindent As an immediate consequence of this definition, we have that $\| \Phi (\bm{a}) \|_{\mathcal{B}, p} \leq \| \Phi \|_{\mathcal{B}, p} \| \bm{a} \|_{\mathcal{B}, p}$ holds for all $\bm{a} \in \mathcal{B}^n \setminus \bfz_\cB$.
%
%In a similar manner, given $1 \leq p \leq \infty$, we can define the norm $\| \cdot \|_{\mathcal{N}, p}$ over $\mathcal{N}$ satisfying a result analogous to Lemma \ref{BNormLemma} by replacing every $\mathcal{B}$ by $\mathcal{N}$ in (\ref{BpNorm}), (\ref{BinfNorm}), and Definition \ref{BopNorm}.
%
%
%\subsection{Two's Complement}
%\label{TwoCompSec}
%From the end of Step 2 through the beginning of Step 5, the implementation of ZFP stores the integer components of each block using a normalized fixed-point, two's complement binary integer representation. Given $z \in \mathbb{Z}$, the two's complement representation is of the form
%\begin{align*}
%\text{Two's Complement:} \ \ \ \ z = - t_{N-1} 2^{N-1} + \sum_{i = 0}^{N-2} t_i 2^i,
%\end{align*}
%for some $N \in \mathbb{N}$ and some $t \in \mathcal{C}$. Typically, the
%value of $N$ is chosen beforehand to be the number of bits allotted for
%storing each integer. Unfortunately, this aspect of the two's complement
%representation does not lend itself to a construction of a vector
%space, unlike the vector spaces $\mathcal{B}^n$ and
%$\mathcal{N}^n$ that we constructed in
%Section~\ref{sec:bitvectorSpace}. Thus, instead of working explicitly in
%two's complement, we will take care when defining the operators for Steps 2
%through 5 of ZFP in $\cB^n$ to ensure they mimic the behavior of the
%two's complement representation in the implementation of ZFP. %Note,
%                                %there is a corresponding two's
%                                %complement representation for all $a
%                                %\in \cB$. 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Truncation Operator on $\mathcal{B}^n$ and $\mathcal{N}^n$}\label{ProjectionSubsection}
%In this section, we consider some properties of the trucation operator, $T_{\mathcal{S}}{(\cdot)} $, over the normed vector spaces  $\mathcal{B}^n$ and $\mathcal{N}^n$. The usefulness of these definitions and results will be evident during the analysis of the ZFP compression algorithm in Section \ref{sec:bounds}.
%%%%Note that one natural use for such a map is to take the set $\mathcal{S}$ to be finite. Then the map $F_{\mathcal{B}} P_{\mathcal{S}} F_{\mathcal{B}}^{-1} : \mathbb{R}^n \to \mathbb{R}^n$ returns a finite precision representation of the input. 
%
%\begin{definition}
%\label{def:emaxemin}
%Let $\bm{x} \in \mathbb{R}^n$. The \emph{maximum exponent of $\bm{x}$
%  with respect to $\mathcal{B}$} is 
%\begin{align}
%e_{max, \mathcal{B}}(\bm{x}) = \max_{1 \leq i \leq n} \max_{j} \left\{ j
%\in \mathcal{I} \left( f_{\mathcal{B}}^{-1} \left(\bm{x}_i \right)
%\right) \right\} \label{eqn:emax}, 
%\end{align}
%%%% Commented out old definition: e_{max}(\bx) =  \lfloor \log_2(\max_i{|x_i|})\rfloor
%and \emph{minimum exponent of $\bm{x}$ with respect to $\mathcal{B}$} is
%\begin{align}
%e_{min, \mathcal{B}}(\bm{x}) = \min_{1 \leq i \leq n} \min_{j} \left\{ j \in \mathcal{I} \left( f_{\mathcal{B}}^{-1} \left(\bm{x}_i \right) \right) \right\}, \label{eqn:emin}
%\end{align}
%%%% Commented out old definition: e_{min}(\bx) =  \lfloor \log_2(\min_i{|x_i|})\rfloor, where $\lfloor \cdot \rfloor$ is the floor function.
%provided that the minimum exists. Similarly, we define the \emph{maximum} and \emph{minimum exponent of $\bm{x}$ with respect to $\mathcal{N}$} by replacing $\mathcal{B}$ with $\mathcal{N}$ in (\ref{eqn:emax}) and (\ref{eqn:emin}). 
%\end{definition}
%When it is clear from context which vector $\bm{x}$ is being used and which function $f_{\mathcal{B}}^{-1}$ or $f_{\mathcal{N}}^{-1}$ is used, we will simply write $e_{max}$ and $e_{min}$. The following result provides a relation between elements of $\mathcal{B}$ and $\mathcal{N}$ and $e_{max}$.
%
%\begin{lemma}
%\label{ProjectionLemma1}
%Suppose $\bm{a} \in \cB^n$ and $\bm{d} \in \cN^n$. Then
%\begin{enumerate}
%\item[$(i)$] $\| \bm{a} \|_{\mathcal{B}, \infty} \geq 2^{e_{max, \mathcal{B}}(F_{\mathcal{B}}(\bm{a})))}$.
%\item[$(ii)$] $\| \bm{d} \|_{\mathcal{N}, \infty} \geq \frac{1}{3} 2^{e_{max, \mathcal{N}}(F_{\mathcal{N}}(\bm{d})))}$.
%\end{enumerate}
%\end{lemma}
%\begin{proof}
%$(i)$ follows immediately from the definition of $e_{max, \mathcal{B}}(\bm{x})$. Next, for $z \in \mathbb{Z}$ even we define $\mathcal{J}(z) = \{ 2j \in
%\mathbb{Z} : 2j \leq z\}$ and for $z \in \mathbb{Z}$ odd we define
%$\mathcal{J}(z) = \{ 2j+1 \in \mathbb{Z}:2j+1 \leq z\}$. Letting $e = e_{max, \mathcal{N}}(\bm{x})$, $(ii)$ follows from observing 
%\begin{align*}
%\| \bm{d} \|_{\mathcal{N}, \infty} \geq \left| (-2)^e - \sum_{i \in
%  \mathcal{J}(e-1)} (-2)^{i} \right| = 2^e - \frac{2}{3} 2^e =
%\frac{1}{3} 2^{e_{max, \mathcal{N}}(F_{\mathcal{N}}(\bm{d}))}.
%\end{align*}
%\end{proof}
%
%We now provide a result establishing the relationship between $\bm{a}$
%and $T_{\mathcal{S}} (\bm{a})$ given $\bm{a} \in \mathcal{B}^n$ or
%$\bm{a} \in \mathcal{N}^n$. First note that, for certain choices of $m
%\in \mathbb{Z}$, the constant term $2^{1 - m}$ will regularly occur in
%error bounds established throughout this paper. Hence, we will let
%$\epsilon_m := 2^{1-m}$ for any $m \in \mathbb{Z}$. For example, machine
%epsilon \cite{higham2002accuracy} is defined as $\epsilon_k = 2^{1-k}$
%for precision $k$.  
%
%
%\begin{lemma}
%\label{ProjectionLemma2}
%Suppose $p, q \in \mathbb{Z}$. If $\bm{a} \in \cB^n$ and $\mathcal{S} = \{ i \in \mathbb{Z} : i > p - q \}$ then
%\begin{enumerate}
%\item[$(i)$] $\bm{a} = T_{\mathcal{S}} (\bm{a}) + \Delta \bm{a}$, for some $\Delta \bm{a} \in \mathcal{B}^n$ satisfying $\| \Delta \bm{a} \|_{\mathcal{B}, \infty} \leq \epsilon_q 2^{p}$.
%\end{enumerate}
%Alternatively, if $\bm{d} \in \cN^n$ and $\mathcal{S} = \{ i \in \mathbb{Z} : i > p - q \}$ then 
%\begin{enumerate}
%\item[$(ii)$] $\bm{d} =T_{\mathcal{S}} (\bm{d}) + \Delta \bm{d}$, for some $\Delta \bm{d} \in \mathcal{N}^n$ satisfying $\| \Delta \bm{d} \|_{\mathcal{N}, \infty} \leq \frac{2}{3} \epsilon_q 2^{p}$.
%\end{enumerate}
%\end{lemma}
%\begin{proof}
%Let $1 \leq m \leq n$. Observing 
%\begin{align*}
%\left| f_{\mathcal{B}} \left( \Delta \bm{a}_m \right) \right| = \left| f_{\mathcal{B}} \left( \bm{a}_m - T _{\mathcal{S}} (\bm{a})_m \right) \right| = \sum_{i \in \mathcal{I} \left( \bm{a}_m \ominus T_{\mathcal{S}} (\bm{a})_m \right)} 2^i \leq \sum_{i = -\infty}^{p - q} 2^i = 2^{e - q + 1}
%\end{align*}
%concludes the proof of $(i)$. Next, for $z \in \mathbb{Z}$ even we define $\mathcal{J}(z) = \{ 2j \in
%\mathbb{Z} : 2j \leq z\}$ and for $z \in \mathbb{Z}$ odd we define
%$\mathcal{J}(z) = \{ 2j+1 \in \mathbb{Z}:2j+1 \leq z\}$. Then $(ii)$ follows by observing that  
%\begin{align*}
%\left| f_{\mathcal{N}} \left( \Delta \bm{d}_m \right) \right| = \left|
%f_{\mathcal{N}} \left( \bm{d}_m - T_{\mathcal{S}} (\bm{d})_m \right)
%\right| = \left| \sum_{i \in \mathcal{I} \left( \bm{a}_m \ominus
%  T_{\mathcal{S}} (\bm{a})_m \right)} (-2)^i \right| \leq \left| \sum_{i
%  \in \mathcal{J}(p-q)} (-2)^i \right| = \frac{2}{3} 2^{p -q + 1}. 
%\end{align*}
%\end{proof}
%
%Hence, if $\mathcal{S} = \{ i \in \mathbb{Z} : i > {e_{\max}(F_{\mathcal{B}}(\bm{a}))} - q \}$ then the additional round-off error incurred by the truncation
%operator is dependent on $q$ and the magnitude of the input. Using
%Lemma~\ref{ProjectionLemma2}, we now observe that the component-wise
%relative error introduced by the truncation operator is bounded by 
%\begin{align} 
%\max_{m, f_\cB(\bm{a}_m) \neq 0} f_\cB \left( \left | \frac{\bm{a}_m - T_\cS(\bm{a}_m)}{\bm{a}_m} \right | \right) & \leq \frac{ \left \|\Delta \ba\right \|_{\cB,\infty} }{\min_{m, f_\cB(\bm{a}_m) \neq 0} f_\cB(| \bm{a}_m |)}, \nonumber \\ 
%& =\epsilon_q2^{e_{max}(f_{\mathcal{B}}(\bm{a}))-e_{min}(f_{\mathcal{B}}(\bm{a}))+1},   \label{eqn:componentwiseerror}
%\end{align}
%for $\ba \in \cB^n $ with $F_\cB(\ba) \neq \bfz$. So the component-wise
%error relative to the input is dependent on $q$ and the exponent range, i.e.,
%$\rho =
%e_{max}(F_{\mathcal{B}}(\bm{a}))-e_{min}(F_{\mathcal{B}}(\bm{a}))$. In
%\cite{zfp}, it was noted that in many real-world examples, the exponent
%range was reasonable ($\rho \leq 8$). Thus, depending on $\rho$, $q$
%could be chosen to ensure the component-wise error relative to the input
%remains less than machine epsilon. 
%
%%%% Commented out: Combined this lemma with the one above
%\iffalse
%\begin{lemma}
%\label{ProjectionLemma3}
%Let $\ba \in \{ \bb \in \cN ^n: i\geq 0 \quad \forall i \in \cI(\bb)\}$ and $\beta \in \mathbb{N}_0$ be given. Suppose that $\mathcal{T} = \{ i \in \mathbb{N} : i \geq i_{max} - \beta \}$, where $i_{max} = \max(\cI(\ba))$ . Then
%\begin{align*}
%\bm{a} = T_{\mathcal{T}} (\bm{a}) + \Delta \bm{a},
%\end{align*}
%for some $\Delta \bm{a} \in \mathcal{N}^n$ satisfying $\| \Delta \bm{a} \|_{\mathcal{N}, \infty} \leq 2^{i_{max} - \beta}$ and  $\| \Delta \bm{a} \|_{\mathcal{N}, \infty} \leq 2^{-\beta+1} \| \bm{a} \|_{\mathcal{N}, \infty}$.
%\end{lemma}
%\begin{proof}
%Suppose $1 \leq i \leq n$. Observing that
%\begin{align*}
%\left | f_{\mathcal{N}} \left( \Delta \bm{a}_i \right) \right |&= \left| f_{\mathcal{N}} \left( \bm{a}_i \ominus T_{\mathcal{T}} (\bm{a})_i \right) \right | \\ 
%=& \left | \sum_{j=0}^{i_{max} - \beta-1} a_i(-2)^j  \right |\\ 
%&\leq \sum_{j=0}^{i_{max} - \beta-1} 2^j \\ 
%&\leq 2^{i_{max} - \beta}-1 \\ 
%&\leq  2^{i_{max} - \beta}. \\
%\end{align*}
%concludes the proof of the first claim. 
%Notice, $\|\ba\|_{\cN,\infty} \geq 2^{i_{max}-1}$, then we can conclude the second claim 
%\[ \|\Delta \bm{a} \|_{\cN, \infty} \leq  2^{-\beta +1}\|\ba\|_{\cN,\infty}.\] 
%\end{proof}
%\fi
%%%% End comment out
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Shift Operator on $\mathcal{B}^n$}\label{ShiftSubsection}
%We now wish to determine what can be said about the norm of the shift operator. For $a \in \mathcal{B}$ and $\ell \in \mathbb{Z}$, observe that
%\begin{align*}
%\left| f_\cB(s_{\ell} (a)) \right| = \left| \sum_{i \in \mathcal{I}(a)} 2^{i - \ell} \right| = 2^{-\ell} \left| \sum_{i \in \mathcal{I}(a)} 2^{i} \right| = 2^{-\ell} \left| f_\cB(a) \right|.
%\end{align*}
%This observation, together with the definition of $\| \cdot \|_{\mathcal{B}, p}$, yields the following result pertaining to the norm of the shift operator on the normed vector space $\mathcal{B}^n$.
%
%\begin{lemma}
%\label{ShiftLemma}
%Suppose $\ell \in \mathbb{Z}$ and $1\leq p \leq \infty$. Then $\| S_{\ell} \|_{\mathcal{B}, p} = 2^{-\ell}$ and $\| S_{\ell}^{-1} \|_{\mathcal{B}, p} = 2^{\ell}$.
%\end{lemma}
%%%%I commented this out as it is trivial from the definition of the norm and the observation presented in the beginning of this section.
%\iffalse
%\begin{proof}
%Suppose that $\bm{a} \in \mathcal{B}^n$ with $\bm{a} \neq \bm{0}_{\mathcal{B}}$. Then for $1\leq p <\infty$ we have
%\begin{align*}
%\| S_l (\bm{a}) \|_{\mathcal{B}, p} = \left( \sum_{i = 1}^{n} \left| f_\cB \left(s_l(\bm{a}_i) \right) \right|^p \right)^{1/p} = \left( \sum_{i = 1}^{n} \left| 2^{-l} f_\cB \left( \bm{a}_i \right) \right|^p \right)^{1/p} = 2^{-l} \| \bm{a} \|_{\mathcal{B}, p}
%\end{align*}
%and 
%\begin{align*}
%\| S_l (\bm{a}) \|_{\mathcal{B}, \infty} = \max_{1 \leq i \leq n} \| s_l(\bm{a}_i) \|_{\mathcal{B}} = \max_{1 \leq i \leq n} \left\{ 2^{-l} \| \bm{a}_i \|_{\mathcal{B}} \right\} = 2^{-l} \max_{1 \leq i \leq n} \| \bm{a}_i \|_{\mathcal{B}} = 2^{-l} \| \bm{a} \|_{\mathcal{B}, \infty}.
%\end{align*}
%Hence, $\displaystyle \frac{\| S_l (\bm{a}) \|_{\mathcal{B}, p}}{\| \bm{a} \|_{\mathcal{B}, p}} = 2^{-l}$, for all $1\leq p <\infty$. Since $\bm{a} \in \mathcal{B}^n$ was taken to be arbitrary, we conclude that $\| S_l \|_{\mathcal{B}, p}=2^{-l}.$
%As $S_l^{-1} =S_{-l}$, $\| S_l^{-1}  \|_{\mathcal{B}, p}=2^{l}$ immediately follows. 
%\end{proof}
%\fi
%
%To summarize, we have now constructed the normed vector spaces $\cB^n$
%and $\cN^n$ and bijective maps between $\cB^n$ and $\mathbb{R}^n$ and
%$\cN^n$  and $\mathbb{R}^n$. We can easily represent floating-point or
%fixed-point representations by applying the truncation operator
%$T_\cS{(\cdot)} $ on elements of $\cB^n$ or $\cN^n$, and
%multiplication by powers of two in $\mathbb{R}^n$ is equivalent to
%applying shift operator, $S_{\ell}$, to elements in $\cB^n$ and
%$\cN^n$. The added benefit of these spaces and operators is that they
%allow us to easily define operators for each step of the ZFP compression
%algorithm as described is Section~\ref{sec:zfp}. 
%
%%%%end of commented out proof
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\subsection{Floating-Point and Block-Floating-Point Error}
%%\label{sec:fpandbfp}
%%
%%\todo{I have not spent any time editing this section as I do not think we need the majority of this section (since we will be working primarily in the bit vector space). Once all of the other sections are complete we can see what we still need from this section to get the desired results. I copied the $e_{\max}$ definition to the section on the projection operator as it was needed there for one result.}
%%
%%\begin{gnote}
%%This section might be a bit out of place....  
%%I think it distracts too much from the flow and could be an appendix?
%%Don't move it just yet, as I am not 100\% sure it can be moved cleanly without causing a headache.
%%\end{gnote}
%%
%%%As noted from above, $\cB_m$ represents the bit-vector space that represents a floating-point approximation of a number and is a subset of the field $\cB$. We will represent a value in $\cB $ by the closest approximation in $\cB_m$ and an error term.  First, before we discuss the bit-vector space recall  
%%The information lost at step 2, and 8 of the ZFP compression algorithm is similar to information lost from a floating-point approximation. To help with the analysis, we recall classic floating-point properties and theorems. Let $fl_{\james{m}} (\cdot): \mathbb{R} \rightarrow \mathbb{R}$ be the operator that maps $x\in \mathbb{R}$ to its closest floating-point representation. Let $\epsilon_m$ be machine epsilon for the floating-point approximation with $m$ bits of precision. From \cite{higham2002accuracy}, we have the following lemma. 
%%%Ideally we wish computers cHowever, $\cB_m$ is space that we can work in. However for the analysis we will always assume we are in $\cB$. The operator $T_\cS$ converts the block into its block-floating point representation. In this section we will redefine the operation $T_\cS$ from above. This representation will be useful in Step 2 and Step 8 and is similarly to the floating point relative roundoff error model. We will first discuss the floating point error and then show its similarity with the operator $T_\cS$. 
%%%
%%%Let $p: \mathbb{R} \rightarrow \mathbb{R}$ be the operator that maps $x\in \mathbb{R}$ to its closest floating-point representation. From \cite{higham2002accuracy}, we have the following Lemma about the error. 
%%\begin{lemma}
%%\label{lemma:floatingapprox}(Theorem 2.2 \cite{higham2002accuracy})
%% If $x \in  \mathbb{R}$ and $x$ is in the range of the floating-point approximation then 
%%\[fl\aedit{_m}(x) = x+\delta x, \]
%%\aedit{where $|\delta x| \leq \frac{1}{2}\epsilon_m |x|$.}
%%\end{lemma} 
%%\noindent \aedit{Notice, with the notation derived above, that only $F_B^{-1}(fl_m(x))$ is garenteed to be representable in  $\cB_k$.} 
%%
%%\noindent \jamesremoved{\sout{Notice, with the notation derived above, that $fl(x)$, $x$, $\delta x\in \cB$ and $fl(x) \in \cB_k$.} (no longer relevant as bit-vector space information has been removed. This handles Geoff's concern with the original statement.)}
%%
%%\begin{gnote}
%%How is it that $fl(x),x, \delta x\in \cB$ or $fl(x) \in \cB_k$?   Is this just a typo??   Do you mean $\mathbb{R}$?   Should it be $f_{\cB}(fl(x)) \in \cB_k$ for some $k$ dependent on $m$?   Please fix and ensure it doesn't impact anything below.   Also, decide if $\delta$ is a number in itself, as I cannot tell if the $|\delta| \leq u$ is a typo or not.   If you want to be consistent with what follows, maybe use $\Delta x$ and $|\Delta x| \leq u$?   Note that $\delta$ can be a scalar in 1d and this makes sense, but not in $d\geq 2$.
%%\end{gnote}
%%
%%\jamesremoved{\sout{Lemma \ref{lemma:floatingapprox} can be extended using vector notation,}} \james{Extending $fl$ to be a map from $\mathbb{R}^n$ to $\mathbb{R}^n$ as} \[
%%fl\aedit{_m}(\bx) = \begin{bmatrix} 
%%fl\aedit{_m}(x_1) \\
%%\vdots\\
%%fl\aedit{_m}(x_n) 
%%\end{bmatrix}, \text{ for all } \bx \in \mathbb{R}^n\jamesremoved{\xout{\ .\ }} \] \james{it then follows from Lemma \ref{lemma:floatingapprox} that there exists a vector $\Delta \bm{x} \in \mathbb{R}^n$ with $\| \Delta \bx \|_{\infty} \leq \varepsilon_m$ such that}
%%\[\jamesremoved{\xout{fl(\bx) = \bx+\Delta \bx, \qquad | \gedit{(\Delta \bx)_i} | \leq u ,}} \] 
%%\[ \james{fl\aedit{_m}(\bm{x})_i = \bm{x}_i \left( 1 + \Delta \bm{x}_i \right), \text{ for } 1 \leq i \leq n.} \]
%%\jamesremoved{\sout{component-wise \gedit{for $\forall i$} and}}
%%\begin{equation*} \jamesremoved{\xout{\|\bx - fl(\bx)\|_\infty  = \|\Delta \bx \|_\infty  \leq u \|\bx \|_\infty .}}\end{equation*}
%%\jamesremoved{\sout{A block-floating-point representation can be considered a special case of a floating-point representation.} (The formal definition below should handle Geoff's concerns)}
%%\begin{gnote}
%%I don't think the reader will know what the 'entire block' means or what $n$ is in the sentence below, maybe fix with a reference to the section/figure that explains this.
%%\end{gnote}
%%\james{We now define the notion of a block-floating-point representation.
%%\begin{definition}
%%A \emph{block-floating-point} representation of $\bm{x} \in \mathbb{R}^n$ is a vector $\hat{\bm{x}} \in \mathbb{R}^n$ such that $\hat{\bm{x}}_i = fl_{\nu}(\bm{x}_i)$, for all $1 \leq i \leq n$, where $\nu = e_{\max}(\bm{x}) + 1$.
%%\end{definition}}
%%\jamesremoved{\sout{One exponent will be used for the entire block $\bx \in \mathbb{R}^n$, i.e.,}}
%%\[ \jamesremoved{\xout{\bx = \hat{\bx} \cdot 2^\nu,}} \]
%%\jamesremoved{\sout{where $\hat{\bx} = (\bx \cdot2^{-\nu})$ is the block mantissa.} (This does not seem to be a correct interpretation. According to this definition there is no loss of information in the block-floating-point representation. I understand that $\hat{\bm{x}}$ is supposed to be the block mantissa but when you multiply $\hat{\bm{x}}$ by $2^{\nu}$ you fully recover $\bm{x}$ which is not always the case in the block-floating-point representation.)}
%%\jamesremoved{\sout{The exponent used will be the maximum exponent of the block defined as $\nu := e_{max}+1,$ where}} \hltodo{Note that}
%%\begin{equation} e_{max} := e_{max}(\bx) =  \lfloor \log_\cB(\max_i{|x_i|})\rfloor \label{eqn:emax} \end{equation}
%%\jamesremoved{\sout{and}} \james{where} $\lfloor \cdot \rfloor$ is the floor function. Similarly, we define the minimum exponent of \jamesremoved{\sout{the block}} \james{$\bm{x} \in \mathbb{R}^n$} as 
%%\[e_{min} := e_{min}(\bx) =  \lfloor \log_\cB(\min_i{|x_i|})\rfloor,  \]
%%\hltodo{which will be used later in this section.} \todo{(This definitions bewteen the highlighted regions were moved to a different section.)}
%%\todo{For this section everything up to here has been edited.} 
%%
%%The above roundoff error model used for floating-point can not be applied directly to the block-floating-point representation. Instead, a scaled additive roundoff error model, introduced in \cite{MitrablockRoundingError}, will be used. \aedit{\sout{Define $fl_\nu(\cdot): \mathbb{R}^n \rightarrow \mathbb{R}^n$ as the operator that maps $\bx\in \mathbb{R}^n$ to its closest block-floating-point representation with exponent $\nu$. }}
%%\begin{definition}
%%\label{assmp:bfp}
%%\aedit{If $x_i \in \mathbb{R}$ and $fl_\nu(x_i)$ is the block-floating-point representation with precision $t$, we define the scaled additive error as: }
%%\[fl_\nu(x_i) - x_i = \epsilon_{t} 2^{\nu-1},  \]
%%where $\epsilon_{t}$ is the machine epsilon with respect to precision $t$. 
%%\end{definition}
%%\begin{gnote}
%%Is this the definition of $fl_\nu(\cdot)$?   It's not presented that clearly...
%%\end{gnote}
%%\gedit{
%%Is this true:
%%$$
%%fl_\nu(x_i) := fl(2^{-\nu}x_i)*2^{\nu} 
%%\quad ???
%%$$
%%}
%%\begin{anote}It is true but the operators have different precision. In single, the floating point precision is $m= 24$ and the block-floating-point has $m = 31$. Decided to change the definition without mention of $fl()$. 
%%\end{anote}
%%\noindent \aedit{\sout{Then, $fl_\nu(x_i) - x_i = [fl(\hat{x_i}) - \hat{x_i}]*2^{\nu} = \epsilon_{t} 2^{\nu-1} $ }}
%%
%%\aedit{\sout{holds from Lemma \ref{lemma:floatingapprox}. }} \aedit{Note that $\epsilon_{t}$ is the machine epsilon that is dependent on precision with respect the block-floating-point representation which will differ from the precision when using a floating-point representation, that is $\epsilon_m \neq \epsilon_{t}$. }\aedit{\sout{Thus, the notation $u_\nu$ is used to differentiate from $u$.}} In vector notation, we have 
%%\[ fl_\nu(\bx) = \bx +\Delta_\nu \bx, \qquad |\gedit{(\Delta_\nu \bx)_i}| \leq  \aedit{\epsilon_{t}2^{\nu-1}}  , \gedit{\quad \forall i} .\]
%%and 
%%\begin{equation} \|\bx - fl_\nu(\bx)\|_\infty  = \|\Delta_\nu \bx \|_\infty \leq  \aedit{\epsilon_{t}\|\bx_i\|_\infty}. \label{eqn:flnu} \end{equation}
%%\aedit{\sout {A useful lemma for the analysis with respect to the block-floating-point conversion is provided below. }}
%%\begin{gnote}
%%Do we really need the first lemma?   I didn't see it referenced, and it could just show up in the proof of the second lemma.
%%\end{gnote}
%%
%%\begin{lemma}
%% \label{lemma:norms}
%% \aedit{\sout{ Let $\bx \in \mathbb{R}^n$ such that $\bx \neq \bfz$ and $e_{max}$ be define as in (\ref{eqn:emax}),  then 
%%$2^{e_{max}}\leq \|\bx\|_\infty\leq 2^{e_{max}+1} . $ }}
%%\end{lemma}
%%%\begin{proof}
%%%Follows immediately from $\|\bx\|_\infty  = \max_i|x_i| \geq 2^{e_{max}}$ and $\|\bx\|_\infty  = \max_i|x_i| \leq 2^{e_{max}+1}$.
%%%\end{proof}
%%\begin{lemma} \label{thm:bfpnorm}
%%\aedit{\sout{ Let $\bx \in \mathbb{R}^n$ such that $\bx \neq \bfz$ and $\nu = e_{max}+1$, where $e_{max}$ is defined in (\ref{eqn:emax}) then, 
%%$\| \gedit{\Delta_\nu \bx } \|_\infty \leq \aedit{\epsilon_t} \|\bx\|_\infty.$}}
%%\end{lemma}
%%
%%\begin{proof}
%% \aedit{\sout{Immediately follows from equation (\ref{eqn:flnu}) and $2^{e_{max}}\leq \|\bx\|_\infty\leq 2^{e_{max}+1}$.}}
%%\end{proof}
%%The above bound can be misleading.  If \aedit{$\epsilon_t \leq \epsilon_m$}, the bound implies that the error occurred by the block-floating-point conversion is not any greater what would occur from the floating-point conversion. However, by observing the component-wise relative error, one can see that information is lost if the span of representable numbers for the block is greater than some threshold, i.e, if $\bx \neq \bfz$, then 
%%\aedit{\begin{align} 
%%\max_{i, \bx_i \neq 0} \left |\frac{fl_\nu(\bx_i) - \bx_i}{\bx_i}\right |  & \leq \frac{ \left \|fl_\nu(\bx) - \bx\right \|_\infty }{\min_{i, \bx_i \neq 0}{|\bx_i|}} \\ 
%%& = \epsilon_t 2^{e_{max}-e_{min}+1}.  \label{eqn:componentwiseerror}
%%\end{align}}
%%\begin{gnote}
%%Note that we can have $\bx = {\bf 0}$ and $\min_i{|x_i|} =0$.   Does the previous equation hold in this case?   If not, fix or explain... 
%%\end{gnote}
%%\begin{anote}
%%The above was for the nonzero elements in the block. If $x_i = 0$ no relative error occur. 
%%\end{anote}
%%If $e_{max}-e_{min}$ satisfy \aedit{$\epsilon_t2^{e_{max}-e_{min}+1} \leq \epsilon_m$}, the potential information that might be loss from the block-floating-point conversion is less than error occurred from the floating-point approximation. Otherwise, the component-wise \aedit{relative} error is greater than $\epsilon_m$ and bits are lost from the representation.
%%
%%\begin{gnote}
%%I think there are several thinks that will improve this section: (i) have all results in terms of $\epsilon_m$.   There is no need to introduce $u$ and it is just one-half of $\epsilon_m$.   Clearly present what $u_\nu$ is in terms of $\epsilon_m$. (ii) use formal definition block(s) more purposefully, (iii) Use a formal remark block for the comments at the end of the section so it can be referenced clearly.
%%\end{gnote}
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

